Strong Revenue (Non-)Monotonicity of Single-parameter Auctions

Consider Myerson's optimal auction with respect to an inaccurate prior, e.g., estimated from data, which is an underestimation of the true value distribution. Can the auctioneer expect getting at least the optimal revenue w.r.t. the inaccurate prior since the true value distribution is larger? This so-called strong revenue monotonicity is known to be true for single-parameter auctions when the feasible allocations form a matroid. We find that strong revenue monotonicity fails to generalize beyond the matroid setting, and further show that auctions in the matroid setting are the only downward-closed auctions that satisfy strong revenue monotonicity. On the flip side, we recover an approximate version of strong revenue monotonicity that holds for all single-parameter auctions, even without downward-closedness. As applications, we get sample complexity upper bounds for single-parameter auctions under matroid constraints, downward-closed constraints, and general constraints. They improve the state-of-the-art upper bounds and are tight up to logarithmic factors.

==> app-concentration.tex <==
\section{Proof of Corollary~\ref{cor:bernstein}}
\label{app:concentration}

Letting $X_i = x_i - \bar{x}$ in Bernstein's Inequality (Lemma~\ref{lem:bernstein}), and noting that $0 \le x_i \le 1$ implies $\E X_i^2 = \E x_i^2 - \bar{x}^2 \le \E x_i - \bar{x}^2 = \bar{x}(1-\bar{x})$, we have:
%
\[
    \Pr \bigg[ ~ \bigg\vert ~ \frac{1}{N}\sum_{i=1}^{N} x_i - \bar{x} ~ \bigg\vert \geq t ~ \bigg] \leq 2e^{-\frac{Nt^2}{2\bar{x}(1-\bar{x})+\frac{2}{3}t}}
\]

To ensure that the right-hand-side is at most $\delta$, we need:
%
\[
    t^2 \geq \frac{\big(2\bar{x}(1-\bar{x})+\frac{2}{3}t\big)\ln{\frac{2}{\delta}}}{N}
    ~.
\]

It is easy to verify that letting:
%
\[
    t = \sqrt{\frac{2 \bar{x}(1-\bar{x}) \ln{\frac{2}{\delta}}}{N}} + \frac{\ln{\frac{2}{\delta}}}{N}
    ~,
\]
%
satisfies this inequality, and thus proves Corollary~\ref{cor:bernstein}.


